A GRU-based Mixture Density Network for Data-Driven Dynamic Stochastic Programming

The conventional deep learning approaches for solving time-series problem such as long-short term memory (LSTM) and gated recurrent unit (GRU) both consider the time-series data sequence as the input with one single unit as the output (predicted time-series result). Those deep learning approaches have made tremendous success in many time-series related problems, however, this cannot be applied in data-driven stochastic programming problems since the output of either LSTM or GRU is a scalar rather than probability distribution which is required by stochastic programming model. To fill the gap, in this work, we propose an innovative data-driven dynamic stochastic programming (DD-DSP) framework for time-series decision-making problem, which involves three components: GRU, Gaussian Mixture Model (GMM) and SP. Specifically, we devise the deep neural network that integrates GRU and GMM which is called GRU-based Mixture Density Network (MDN), where GRU is used to predict the time-series outcomes based on the recent historical data, and GMM is used to extract the corresponding probability distribution of predicted outcomes, then the results will be input as the parameters for SP. To validate our approach, we apply the framework on the car-sharing relocation problem. The experiment validations show that our framework is superior to data-driven optimization based on LSTM with the vehicle average moving lower than LSTM.

==> Case-Study.tex <==
\section{Experiment Validation}

\subsection{Experiment Setting}
To simulate the profitability of demand optimization, we used taxi operation data from 2006 to 2018 in New York City. The LSTM models are implemented using Python 3.7 under the platform CUDA 10.2 GPU, 16GB RAM, Ubuntu 18.04. The entire data set contains more than 22 million taxi trip records, because huge amount of data set is always beneficial to get better performance using deep learning models. To model LSTM, we split the total data set by train and validation data set. We first separate a test set by selecting the data after 2016-06-01. The training and validation data set are further separated from the data before 2016-6-1 so that the time order is preserved. The features for training models includes latitudes and longitudes for both pickup and drop-off locations, as well as pickup time stamp and number of passengers. These features are necessary for a taxi dispatching system when a passenger call for a demand. First, we hope to build predictive models to estimate the taxi duration trip. In the historical training data, the taxi trip duration is known and therefore the target variable for this task. Although the online APIs such as google map can estimate the taxi trip duration by calculate the distance between the pick-up and drop-off coordinates, it is not automation processing for a dispatching system, and moreover, the taxi trip duration depends on many other factors such as the traffic jam affected by time stamps, the road conditions and so on. The GRU-MDN are implemented using Python 3.7 under the platform CUDA 10.2 GPU, 16GB RAM, Ubuntu 18.04, the mathematical models are solved by Gurobi \footnote{https://www.gurobi.com/downloads/gurobi-software/} 9.0 academic version under the platform Intel i7, 32GB RAM, Windows 10.


The charing station information can be found from \footnote{https://data.ny.gov/Energy-Environment/Electric-Vehicle-Charging-Stations-in-New-York/7rrd-248n} 


The EVDP can be formulated as follows.

$$
\text{maximize} \sum_{t \in T} \sum_{v \in V} \sum_{q \in Q} x_{v q t} d_{q}-\lambda \sum_{t \in T} \sum_{v \in V} t w_{v t}
$$


\subsection{Performance Measures}


==> Related-Work.tex <==
\section{Related work (literature review)}



% \section{Methodology}

% \subsection{Long-Short Term Memory}

% for time-series prediction

\subsection{Gaussian Mixture Model}



The standard GMM can be stated as follows.
$$
p(\boldsymbol{x})=\sum_{k=1}^{K} \pi_{k} \mathcal{N}\left(\boldsymbol{x} | \boldsymbol{\mu}_{k}, \mathbf{\Sigma}_{k}\right)
$$

Given a GMM, the goal is to maximzie the likelihood function with respect to the parameters.

The Expectation-Maximization (EM) algorithm \cite{} is used in maximum likelihood estimation where the problem involves two sets of random variables of which one, X, is observable and the other, Z, is hidden. The goal of the algorithm is to find the parameter vector $\Phi$. The algorithm basically involves two steps: Expectation step and Maximization step which can be summarized as follows.


\par
E-step : $\mathcal{Q}\left(\Phi | \Phi^{l}\right)=E\left[\mathcal{L}_{c}(\Phi | \mathcal{X}, \mathcal{Z}) | \mathcal{X}, \Phi^{l}\right]$
\par
M-step : $\Phi^{l+1}=\arg \max _{\Phi} \mathcal{Q}\left(\Phi | \Phi^{l}\right)$

\par
asdf
\par
asdf
\par
asdf


\begin{algorithm}
\caption{EM algorithm}\label{euclid}
\label{al}
\hspace*{\algorithmicindent} 
\textbf{Input: data $\mathcal{X}$, number of Gaussian $\mathcal{K}$}  
\\
\hspace*{\algorithmicindent} 
\textbf{Output: the parameters of GMM ($\pi$, $\mu$, $\sigma^{2}$)}

\begin{algorithmic}[1]
%\Output{1}{}

\State Initialize the means $\mu_{k}$, variances $\sigma^{2}_{k}$ and mixing coefficients $\pi_{k}$, and evaluate the initial value of the log likelihood.

\State $\boldsymbol{E-step}$
$$
\gamma\left(z_{n k}\right)=\frac{\pi_{k} \mathcal{N}\left(\mathbf{x}_{n} | \boldsymbol{\mu}_{k}, \mathbf{\Sigma}_{k}\right)}{\sum_{j=1}^{K} \pi_{j} \mathcal{N}\left(\mathbf{x}_{n} | \boldsymbol{\mu}_{j}, \mathbf{\Sigma}_{j}\right)}
$$

\State $\boldsymbol{M-step}$

$$
\boldsymbol{\mu}_{k}^{\mathrm{new}} =\frac{1}{N_{k}} \sum_{n=1}^{N} \gamma\left(z_{n k}\right) \mathbf{x}_{n} 
$$

$$
\mathbf{\Sigma}_{k}^{\mathrm{new}} =\frac{1}{N_{k}} \sum_{n=1}^{N} \gamma\left(z_{n k}\right)\left(\mathbf{x}_{n}-\boldsymbol{\mu}_{k}^{\mathrm{new}}\right)\left(\mathbf{x}_{n}-\boldsymbol{\mu}_{k}^{\mathrm{new}}\right)^{\mathrm{T}}
$$

$$
\pi_{k}^{\mathrm{new}} =\frac{N_{k}}{N} 
$$


\State Evaluate the log likelihood

$$
\ln p(\mathbf{X} | \boldsymbol{\mu}, \mathbf{\Sigma}, \boldsymbol{\pi})=\sum_{n=1}^{N} \ln \left\{\sum_{k=1}^{K} \pi_{k} \mathcal{N}\left(\mathbf{x}_{n} | \boldsymbol{\mu}_{k}, \boldsymbol{\Sigma}_{k}\right)\right\}
$$


%\EndOutput
\end{algorithmic}
\end{algorithm}








